Intelligent Autonomous Intersection Management

Connected Autonomous Vehicles will make autonomous intersection management a reality replacing traditional traffic signal control. Autonomous intersection management requires time and speed adjustment of vehicles arriving at an intersection for collision-free passing through the intersection. Due to its computational complexity, this problem has been studied only when vehicle arrival times towards the vicinity of the intersection are known beforehand, which limits the applicability of these solutions for real-time deployment. To solve the real-time autonomous traffic intersection management problem, we propose a reinforcement learning (RL) based multiagent architecture and a novel RL algorithm coined multi-discount Q-learning. In multi-discount Q-learning, we introduce a simple yet effective way to solve a Markov Decision Process by preserving both short-term and long-term goals, which is crucial for collision-free speed control. Our empirical results show that our RL-based multiagent solution can achieve near-optimal performance efficiently when minimizing the travel time through an intersection.

==> tex/reward_sup1.tex <==
\pgfplotstableread[col sep = comma]{figures/reward_11.csv}\rewarddata
\pgfplotstableread[col sep = comma]{figures/reward_15.csv}\rewarddatamd
\pgfplotstableread[col sep = comma]{figures/reward_16.csv}\rewarddatanine
\pgfplotstableread[col sep = comma]{figures/reward_18.csv}\rewarddataninefive

\pgfplotstableread[col sep = comma]{figures/reward_1_11.csv}\rewardonedata
\pgfplotstableread[col sep = comma]{figures/reward_1_15.csv}\rewardonedatamd
\pgfplotstableread[col sep = comma]{figures/reward_1_16.csv}\rewardonedatanine
\pgfplotstableread[col sep = comma]{figures/reward_1_18.csv}\rewardonedataninefive

\pgfplotstableread[col sep = comma]{figures/reward_2_11.csv}\rewardtwodata
\pgfplotstableread[col sep = comma]{figures/reward_2_15.csv}\rewardtwodatamd
\pgfplotstableread[col sep = comma]{figures/reward_2_16.csv}\rewardtwodatanine
\pgfplotstableread[col sep = comma]{figures/reward_2_18.csv}\rewardtwodataninefive

\begin{figure*}[]
\begin{subfigure}{\columnwidth}
\begin{tikzpicture}
\begin{axis}[
xtick={100000, 200000, 300000, 400000, 500000},
height=6cm,
width=8cm,
xmax=360000,
label style={font=\footnotesize},
%every axis x label/.style={at={(current axis.south west)}, left=0mm, above=-6mm},
ylabel={$r_1 + r_2$},
xlabel={steps},
legend style={
legend cell align={left},
legend pos=south east,
font=\small,
legend image post style={xscale=0.5}
}
]
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewarddata};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewarddatanine};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewarddataninefive};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewarddatamd};

%\addplot table [x=item, y=noLA, col sep=comma]{\lanedata};

 

\legend{DQN-1, DQN-0.9, DQN-0.95, MD-DQN}
\end{axis}
\end{tikzpicture}
     \centering
     \caption{Total episodic reward: ($r_1 + r_2$)}
     \label{fig:total reward}
\end{subfigure}

\begin{subfigure}{\columnwidth}
\begin{tikzpicture}
\begin{axis}[
xtick={100000, 200000, 300000, 400000, 500000},
height=6cm,
width=8cm,
xmax=360000,
label style={font=\small},
%every axis y label/.style={at={(current axis.north west)}, left=-2mm, above=2mm},
ylabel={$r_2$},
xlabel={steps},
legend style={
legend cell align={left},
legend pos=south east,
font=\scriptsize
}
]
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardtwodata};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardtwodatanine};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardtwodataninefive};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardtwodatamd};

%\addplot table [x=item, y=noLA, col sep=comma]{\lanedata};

 

%\legend{DQN-1, DQN-0.9, MD-DQN}
\end{axis}
\end{tikzpicture}
     \centering
     \caption{Cruise control reward ($r_2$)}
     \label{fig:cruise reward}
\end{subfigure}

\begin{subfigure}{\columnwidth}
\begin{tikzpicture}
\begin{axis}[
xtick={100000, 200000, 300000, 400000, 500000},
height=6cm,
width=8cm,
xmax=360000,
label style={font=\small},
%every axis y label/.style={at={(current axis.north west)}, left=-2mm, above=2mm},
ylabel={$r_{1,end}$},
xlabel={steps},
legend style={
legend cell align={left},
legend pos=south east,
font=\scriptsize
}
]
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardonedata};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardonedatanine};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardonedataninefive};
\addplot table [mark=none, x=Step, y=Smoothed Value, col sep=comma]{\rewardonedatamd};

%\addplot table [x=item, y=noLA, col sep=comma]{\lanedata};

 

%\legend{DQN-1, DQN-0.9, MD-DQN}
\end{axis}
\end{tikzpicture}
     \centering
     \caption{Trj. control reward (at the end of episode)}
     \label{fig:trajectory reward}
\end{subfigure}
\vspace{-3mm}
\caption{The reward (the moving average with window size 10) achieved through fixed discount Q-learning and multi-discount Q-learning in I-AIM.}
\label{exp-mulit-discount}
\vspace{-4mm}
\end{figure*}

